Stable Marriage Matching for Traffic-Aware Space-Air-Ground Integrated Networks: A Gale-Shapley Algorithmic Approach

In keeping with the rapid development of communication technology, a new communication structure is required in a next-generation communication system. In particular, research using High Altitude Platform (HAP) or Unmanned Aerial Vehicle(UAV) in existing terrestrial networks is active. In this paper, we propose matching HAP and UAV using the Gale-Shapley algorithm in a relay communication situation. The numerical simulation results demonstrate that applying the Gale-Shapley algorithm shows superior performance compared to random matching.

==> simulation/parameters.tex <==
필요한 파라미터

1. UAV U = {u1, u2, ... um}
	좌표공간 크기: 10km * 10km * 300m , 고도: 지상에서 50~350m 사이
    Deployment: 위 공간 내에 random하게 1000개 배치
    각 UAV가 서비스하는 장치의 수: 0~9 사이의 random한 수
    
2. HAP H = {h1, h2, ...hn }
	좌표공간 크기: 5km * 5km * 1km, 고도: 지상에서 20~21km 사이
    Deployment: 위 공간 내에 random하게 200개 배치
    각 h는 최대 UAV 5개와 매칭 가능
    
3. Matching M = {(h^i_n, um)}
  매칭 기준: 거리가 가까운 UAV, 서비스해주는 유저가 많은 UAV
  
 순위를 매기기 위한 기준 :   UAV가 서비스해주는 인원수 / 각 HAP와의 거리

각 HAP는 저마다 자신과 모든 UAV 1000개와의 거리를 계산하고, 기준을 계산한 뒤 순위를 매김

다들 각자의 1-5순위와 matching을 하고 싶겠지만, 그렇지 않은 경우가 분명 존재할 것

이때는 UAV도 HAP 200개에 대한 순위가 있을 테고, 이는 거리만을 고려하게 될 것. 

UAV는 두 HAP를 비교해서 더 가까이 있는 HAP와 엮여있는 거면 새 오퍼를 거절, 더 먼 HAP와 엮여있는거면 기존의 matching을 끊고 새 HAP와 연결

모든 UAV가 연결이 잡힐 때까지 반복

	
    
